chrKanren: Constraint Handling Rules in a Relational Language

We present chrKanren, a dialect of the purely relational constraint logic programming language miniKanren which includes support for Constraint Handling Rules (CHR), a language for writing rule-based programs such as constraint solvers. We show how to integrate CHR's constraint propagation mechanism into the language of miniKanren search streams such that both processes remain complete. We also use chrKanren to illustrate novel applications of constraints in miniKanren, such as semantic unification of user-defined data structures and type-and-example-directed synthesis for relational interpreters in the style of MYTH.

==> eptcsdata.tex <==
\providecommand{\firstpage}{416}
\providecommand{\publicationstatus}{W. Faber, L. Giordano, R. Rocha, V. Santos Costa (Eds.):\\ 42nd International Conference on Logic Programming (ICLP 2026)\\
EPTCS 450, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{https://dx.doi.org/10.4204/EPTCS.450.30}{10.4204/EPTCS.450.30}}

